A Comparative Study on Collecting High-Quality Implicit Reasonings at a Large-scale

Explicating implicit reasoning (i.e. warrants) in arguments is a long-standing challenge for natural language understanding systems. While recent approaches have focused on explicating warrants via crowdsourcing or expert annotations, the quality of warrants has been questionable due to the extreme complexity and subjectivity of the task. In this paper, we tackle the complex task of warrant explication and devise various methodologies for collecting warrants. We conduct an extensive study with trained experts to evaluate the resulting warrants of each methodology and find that our methodologies allow for high-quality warrants to be collected. We construct a preliminary dataset of 6,000 warrants annotated over 600 arguments for 3 debatable topics. To facilitate research in related downstream tasks, we release our guidelines and preliminary dataset.

==> table/iaa.tex <==
\begin{table}[t]
    \small
    \begin{tabularx}{\columnwidth}{X c c c c}
    \toprule%
    \mytab{\textbf{Topic: We should}} & $\alpha$ & $\kappa$ & A1 & A2\\
    \midrule%
    Abolish zoos & 0.64 & 0.42 & 1.60 & 1.50\\
    Intro. compulsory voting & 0.45 & 0.34 & 1.46 & 1.55\\ 
    Ban whaling & 0.63 & 0.41 & 1.49 & 1.25\\
    \midrule%
    Overall & 0.57 & 0.39 & 1.51 & 1.43\\
    \bottomrule
    \end{tabularx}
    \caption{Topic-wise quality statistics for Warr6k dataset. $\alpha$ and $\kappa$ are the Krippendorff's and Cohen's inter-annotator agreement scores, respectively. A1 and A2 are the average scores given to the warrants by our two expert annotators.}
    \label{tab:iaa}
\end{table}

